Forward Invariance of Sets for Hybrid Dynamical Systems (Part II)

This article presents tools for the design of control laws inducing robust controlled forward invariance of a set for hybrid dynamical systems modeled as hybrid inclusions. A set has the robust controlled forward invariance property via a control law if every solution to the closed-loop system that starts from the set stays within the set for all future time, regardless of the value of the disturbances. Building on the first part of this article, which focuses on analysis (Chai and Sanfelice, 2019), in this article, sufficient conditions for generic sets to enjoy such a property are proposed. To construct invariance inducing state-feedback laws, the notion of robust control Lyapunov function for forward invariance is defined. The proposed synthesis results rely on set-valued maps that include all admissible control inputs that keep closed-loop solutions within the set of interest. Results guaranteeing the existence of such state-feedback laws are also presented. Moreover, conditions for the design of continuous state-feedback laws with minimum point-wise norm are provided. Major results are illustrated throughout this article in a constrained bouncing ball system and a robotic manipulator application.

==> Sections/7-BBall.tex <==
\chai{
We demonstrate our main results in a constrained mechanical system with control inputs; namely, a bouncing ball moving vertically that is controlled by impacts on a controlled surface at zero height.
In addition, we attach one end of a nonelastic string with length $\hmax$ to zero height and the other end to the ball; see Figure~\ref{fig:bball} for system configuration.

\IfConf{
	\setlength{\unitlength}{0.2\textwidth}
}{
	\setlength{\unitlength}{0.4\textwidth}}
\begin{figure}[h]
	\centering
	\includegraphics[width= \unitlength]{BouncingBall.eps}
	\put(-1.1,1.3){$x_1= \hmax$}
	\put(-0.5,1){$x_2$}
	\put(-0.45,0.35){String}
	\put(-0.9, 0.5){$\hmin$}
	\caption{Bouncing ball system configuration.}
	\label{fig:bball}
\end{figure}

Compared to a typical bouncing ball system \cite[Example 1.1]{65}, the model considered here has an additional ``pulling phase'' when the ball reaches the height $\hmax$ with possibly nonzero velocity.
The possible pulls from the string at height $\hmax$ and the impacts between the ball and the controlled surface both lead to jumps of the state.
In addition to assuming unitary mass of the ball and negligible weight of the string, forces, and friction, we consider the following:
\begin{enumerate}[label = C\arabic*)]
	\item at impacts with the controlled surface, the uncertain coefficient of restitution is within the range $[e_1, e_2]$, where $0 < e_1 < e_2 < 1$;
	\item\label{item:string} the string breaks when the ball pulls with velocity larger than $\vmax$;
	\item at pulls of the string, the restitution coefficient is $\ep \in (0, 1]$.
%	position of the ball remains the same while its velocity is reset using a restitution law with constant coefficient of 
\end{enumerate}

With $x = (x_1, x_2) \in \reals^2$, $x_1$ and $x_2$ model the height (position) and velocity of the ball, respectively.
Then, with gravity constant $\gamma > 0$, the flow map is defined on $\reals_{\geq 0} \times \reals$ and is given by\footnote{Note that since there are no disturbances and inputs for flow, we omit the subscripts for $f$ and $C$ in this model.}
\ConfSp{\Space}
\begin{align}\label{eq:BpFlowM}
	f(x) := (x_2, -\gamma).
\end{align}
To formulate the flow and jump set, we define a function $E: \reals^2 \rightarrow \reals$ that describes the total energy of the system:
\begin{align}\label{eq:BpE}
	E(x) = \frac{x_2^2}{2}  + \gamma x_1 & \forall x \in \reals^2.
\end{align}
According to \ref{item:string}, the string remains attached to the ball when $x_1 \in [0, \hmax]$ and $x_2 \leq \vmax$, i.e., $E(x) \leq \Emax$ with $\Emax := E(\hmax, \vmax)$.
After impacts with the controlled surface, the ball position $x_1$ remains unchanged, while the velocity $x_2$ is updated to a function of the disturbance $w_d \in \Wd :=[e_1, e_2]$, which represents the uncertain coefficient of restitution, and input $u_d \in \Ud :=[0, \umax]$ with $\umax = \sqrt{2 \Emax}$, which represents the velocity change caused by the controlled surface.
Hence, we model impacts between the ball and the controlled surface as $x_1 = 0$ as
\begin{align}\label{eq:BpJumpM1}
	G_1(x,u_d, w_d) : = (x_1, u_d - w_dx_2)
\end{align}
when $x_2  \leq 0$.
Before every impact $x_2$ is nonpositive, after each impact the ball velocity is updated according to $G_1$.
Then, with a small positive constant $\delta_p < \vmax$, the map
\begin{align}\label{eq:BpJumpM2}
	G_2(x) : = (x_1, \min\{- \ep x_2, -\delta_p\})
\end{align}
models the pulls between the ball and the string when $x_1 = \hmax$ and $x_2 \in [0, \vmax]$.
Since before every pull $x_2$ is nonnegative, after each pull the ball velocity reverses its sign and updates according to $G_2$.
Note that since closed jump sets are preferred as suggested in \ref{item:A1} of Definition~\ref{def:hbc}, we only allows the $x_2$ component to jump to a strictly negative value that is lower bounded (and controllable) by $-\delta_p.$

Then, the hybrid system $\Huw = (C,f,\Duw,\Guw)$ with control input $u_d$ and disturbance $w_d$ has state $x$ and dynamics on space ${\cal X} = \reals^2 \times\Ud \times \Wd$ that is given by
\begin{align}\label{eq:Bplant}
	\dot{x} &= f(x) &x&\in C,\\
	x^+ &= \Guw(x,u_d, w_d) &(x, u_d, w_d) &\in \Duw,
\end{align}
where the flow set $C$ is given by
\begin{align}\label{eq:BC}
	C: = \{x \in \reals^2 : 0 \leq x_1 \leq \hmax, E(x) \leq \Emax\},
\end{align}
and the jump set $\Duw$ is given by $\Duw: = D_1 \cup D_2$ with
\begin{align}\label{eq:BD}
	&D_1: =\{(x,u_d, w_d) \in {\cal X} : x_1 = 0, x_2 \in [-\sqrt{2\Emax}, 0]\},\\
	&D_2 :=\{(x,u_d, w_d) \in {\cal X} : x_1 = \hmax, x_2 \in [0, \vmax]\},
\end{align}
where the jump map $\Guw$ is given by
\begin{align}\label{eq:BG}
	\Guw(x,u_d, w_d) : =
	\begin{cases}
		G_1(x,u_d, w_d) &  \ifeq (x,u_d, w_d) \in D_1\\
		G_2(x) &  \ifeq (x,u_d, w_d) \in D_2.
	\end{cases}
\end{align}

We have the following control design goal: under the presence of disturbances $w_d$, control the ball at impacts so that when the ball has initial condition $x(0,0) = (x_1(0,0), x_2(0,0))$ with $x_1(0,0) \in [\hmin, \hmax]$ and $E(x(0,0)) \in [0,\Emax]$, the string remains attached to the ball, and the peak height of the ball after each bounce is at least $\hmin$.
This objective is achieved by rendering the set
\begin{align}\label{eq:BK}
	\K = L_\Ly(-\gamma \hmin) \cap (C \cup \Pd{\Duw})
\end{align}
robustly controlled forward invariant for $\Huw$, where $\Ly(x) : = -E(x)$ for every $x \in C\cup \Pd{\Duw}$.

Given system parameters $e_1, e_2, e_p, \vmax$ and $\hmax$, the control goal can be achieved for $\hmin$ such that $\sqrt{\gamma\left(\hmin + \frac{\varepsilon}{2}\right)} < e_1 \sqrt{\Emax}$ and with $\varepsilon > 0$,
\begin{align}\label{eq:epsilon}
	\gamma(\hmin + \varepsilon) \leq \frac{(1 +e_1 - e_2)^2}{2}\Emax.
\end{align}
Since the control input appears in the map $G_1$ only, for every $x \in \Pd{D_1}$, according to \eqref{eq:rld}, the set $\Ld$ in \eqref{eq:rld} is given by
\begin{align}\label{eq:BLd}
	\Ld(x) = [0, \sqrt{2\Emax} + e_2x_2].
\end{align}
In fact, $\Ld$ collects all control input values $u_d$ such that $G_1(x,u_d, w_d) \in C \cup \Pd{\Duw}$ for all $w_d \in [e_1, e_2]$; i.e., every such $u_d$ is such that $E(0, G_1(x, u_d, e_2)) \leq \Emax$.
Then, since $\Md = \{0\} \times [-\sqrt{2\Emax}, -\sqrt{\gamma \hmin}]$ and $\uxd(x) = \Ud$, \ref{item:weakExist1} in Theorem~\ref{thm:weakExist} holds for $\Huw$.
Now, consider the constant $\rU = -\gamma(\hmin - \varepsilon)$ and the function $\rd$ defined as $\rd(x)  = \gamma \varepsilon$ for every $x \in \Ls$.
We show that the pair $\clfpair$ defines a RCLF for forward invariance as in Definition~\ref{def:rclf}.
First, \eqref{eq:Rly1} and \eqref{eq:ly1} hold on $C$  since, for every $x \in C$,
\begin{align}\label{eq:BVdot}
	\inner{\nabla \Ly(x)}{f(x)} = -x_2(-\gamma) - \gamma x_2 = 0.
\end{align}
Then, we show the pair $\clfpair$ is such that \eqref{eq:CLF-D} holds for constant $\level = -\gamma\hmin < \rU$.
Moreover, for every $x \in \Ls \cap \Pd{D_1}$, we have
\begin{align*}
	\min\limits_{u_d \in \Ld(x)} &\max\limits_{w_d \in [e_1,e_2]} \Ly(G_1(x,u_d, w_d))\\
	&= \min\limits_{u_d \in \Ld(x)} \max\limits_{w_d \in [e_1,e_2]} \left\{- \frac{(u_d - w_dx_2)^2}{2} \right\}\\
	&= - \frac{(\sqrt{2\Emax} + e_2x_2 - e_1x_2)^2}{2}
\end{align*}
Since $x_2 \in [-\sqrt{2\Emax}, -\sqrt{2\gamma\hmin}]$ and condition \eqref{eq:epsilon}, we have
\begin{align*}
	\min\limits_{u_d \in \Ld(x)} &\max\limits_{w_d \in [e_1,e_2]}  \Ly(G_1(x,u_d, w_d)) + \rd(x)\\
	&\leq  - \frac{(\sqrt{2\Emax} + (e_2 - e_1)(-\sqrt{2\Emax}))^2}{2} + \rd(x)\\
	&= - \frac{(1+e_1-e_2)^2}{2}\Emax + \gamma \varepsilon
	\leq -\gamma \hmin = \level
\end{align*}
For every $x \in \Ls \cap \Pd{D_2}$, we have $x_2 \in [0, \vmax]$ and
\IfConf{
	\begin{align}\label{eq:Bg2}
	\hspace{-5mm}
	\begin{split}
	\min\limits_{u_d \in \Ld(x)} \max\limits_{w_d \in [e_1,e_2]} & \Ly(G_2(x))\\
	&= - \frac{(\min\{- \ep x_2, -\delta_p\})^2}{2} -\gamma \hmax < \level.
	\end{split}
	\end{align}
}{
\begin{align}\label{eq:Bg2}
	\hspace{-5mm}
	\begin{split}
		\min\limits_{u_d \in \Ld(x)} \max\limits_{w_d \in [e_1,e_2]}  \Ly(G_2(x))
		= - \frac{(\min\{- \ep x_2, -\delta_p\})^2}{2} -\gamma \hmax < \level.
	\end{split}
\end{align}
}
Hence, the pair $\clfpair$ defines a robust control Lyapunov function for forward invariance for $\Huw$ according to Remark~\ref{rem:relax} and Definition~\ref{def:rclf}.

Next, following the steps in Section~\ref{sec:design}, we construct the regulation map $\Gamma_d.$
Since there is no control input during flows, we omit defining $\Gamma_c$.
Moreover, the input $u_d$ is only active when $(x, u_d, w_d) \in D_1$, we define the selection map $\Gamma_d$ based on $G_1$ only.
Then, for $\level = -\gamma\hmin$ and for every $(x, u_d) \in \{(x, u_d) \in \reals^2 \times \Ud: (x, u_d, w_d) \in (\Ls \times \Ud \times \Wd) \cap D_1\}$, with $\sigma = \frac{1}{2}$, $\Gamma_d$ is given by
\begin{align*}
	\Gamma_d(x, u_d)
	&= \max\limits_{w_d \in [e_1, e_2]} \Ly(G_1(x, u_d, w_d)) + \frac{\rd(x)}{2} - \level\\
	&= -\frac{(u_d - e_1x_2)^2}{2} + \gamma \left(\frac{\varepsilon}{2} + \hmin\right).
\end{align*}
Item \ref{item:weakExist2} in Theorem~\ref{thm:weakExist} holds since the function $u_d \mapsto \Gamma_d(x, u_d)$ is convex on $\Ld(x)$ for each $x \in \Md$.
For each $x \in \reals^2$, the map $S_d$ in \eqref{eq:Sc} is given by
\begin{align}\label{eq:BSd}
	\hspace{-5mm}
	S_d(x) : =
	\begin{cases}
		\{u_d \in \Ld(x): &\!\!\!\! \gamma (\frac{\varepsilon}{2} + \hmin) -\frac{(u_d - e_1x_2)^2}{2} < 0\} \\
		&\ifeq x \in \Ls \cap \Pd{D_1}, \\
		\reals & \otherw.
	\end{cases}
\end{align}
In addition, $\Huw$ given in \eqref{eq:Bplant} satisfies conditions \ref{item:A1p} - \ref{item:A3p} in Lemma~\ref{lem:hbc}.
According to Theorem~\ref{thm:weakExist}, there exists a state feedback $\kd : \reals^2 \rightarrow \reals$ that is continuous on $\Md$.
In particular, such a feedback is selected from the closure of map $S_d$ given in \eqref{eq:BSd}, which reduces to an interval:
\IfConf{
	\begin{align}\label{eq:BSdcl}
	\overline{S_d}(x): = \left[\max\left\{\sqrt{2\gamma\left(\frac{\varepsilon}{2} + \hmin\right) } + e_1x_2,0\right\},\right.\\
	\left. \sqrt{2\Emax} + e_2x_2\right].
	\end{align}
}{
\begin{align}\label{eq:BSdcl}
	\overline{S_d}(x): = \left[\max\left\{\sqrt{2\gamma\left(\frac{\varepsilon}{2} + \hmin\right) } + e_1x_2,0\right\}, \sqrt{2\Emax} + e_2x_2\right].
\end{align}
}
%which implies, when $x\in \Pd{D_1}$, $G_1(x, \kd(x), e_1) \geq \sqrt{2\gamma(\chai{\frac{\varepsilon}{2}} + \hmin)}$ and $\kd(x) \in \Ld(x)$ given in \eqref{eq:BLd}.
One such continuous selection is %$\kd(x) : = x_2 + \sqrt{2\Emax}$, another is
\begin{align}\label{eq:Bkd}
	\kd(x) : = \sqrt{\frac{\gamma(\frac{\varepsilon}{2} + \hmin)}{\Emax}}x_2 + \sqrt{2\gamma\left(\frac{\varepsilon}{2} + \hmin\right)}.
\end{align}

Since Corollary~\ref{coro:rcFI} provides conditions guaranteeing robust controlled forward invariance for hybrid systems without a Lyapunov function, we verify that our design of $\kd$ in \eqref{eq:Bkd} indeed renders $\Mr$ robustly controlled forward invariant for $\Huw.$
To this end, first, $\K$ is a subset of $C \cup \Pd{\Duw}$, $F$ is Lipschitz and $F(x)$ is convex on $C$ by construction and \ref{item:rcFI4} holds since $\K \cap C$ is compact.
Then, item \ref{item:rcFI1} and \ref{item:rcFI5} hold true trivially; while item \ref{item:rcFI3} holds since \eqref{eq:BVdot} and item 1) of Lemma~\ref{lem:innerTcone}.
Finally, for the closed-loop system with $u_d$ replaced by $\kd$ in \eqref{eq:Bkd}, we check the extreme cases for every $x \in \K \cap \Pd{D_1}$ and every $x \in \K \cap \Pd{D_2}$.
More precisely, the worst case for impact with zero height is $x_2 = - \sqrt{2\gamma\hmin}$ before the impact and $x_2$ is updated by map $G_1(x, \kd(x), e_1)$, i.e.,
\IfConf{
	\begin{align}
	G_1&(x, \kd(x), e_1)\\
	&= \sqrt{\frac{\gamma\left(\frac{\varepsilon}{2} + \hmin\right)}{\Emax}}x_2 + \sqrt{2\gamma\left(\frac{\varepsilon}{2} + \hmin\right)} - e_1x_2\\
	&= \sqrt{2\gamma\left(\frac{\varepsilon}{2} + \hmin\right)} + \\
	& \quad \left(\sqrt{\frac{\gamma\left(\frac{\varepsilon}{2} + \hmin\right)}{\Emax}} - e_1\right)(- \sqrt{2\gamma\hmin}),
	\end{align}
}{
\begin{align}
	G_1(x, \kd(x), e_1)
	&= \sqrt{\frac{\gamma\left(\frac{\varepsilon}{2} + \hmin\right)}{\Emax}}x_2 + \sqrt{2\gamma\left(\frac{\varepsilon}{2} + \hmin\right)} - e_1x_2\\
	&= \sqrt{2\gamma\left(\frac{\varepsilon}{2} + \hmin\right)} + \left(\sqrt{\frac{\gamma\left(\frac{\varepsilon}{2} + \hmin\right)}{\Emax}} - e_1\right)(- \sqrt{2\gamma\hmin}),
\end{align}
}
which is greater than $\sqrt{2\gamma\left(\frac{\varepsilon}{2} + \hmin\right)}$ since $\sqrt{\gamma\left(\frac{\varepsilon}{2} + \hmin\right)} < e_1 \sqrt{\Emax}$.
Then, \ref{item:rcFI2} holds for every $x \in \K \cap \Pd{D_2}$ since \eqref{eq:Bg2}.

Simulations are generated to show solutions to $\Huw$ controlled by $\kd$ in \eqref{eq:Bkd} with system parameters
$\gamma = 9.81, \hmin = 10, \hmax = 12, \vmax = 6\sqrt{\gamma}, e_1 = 0.8, e_2 = 0.9, e_p = 0.95, \varepsilon = 0.1$, and $\delta_p = 0.01.$\footnote{All simulations in this section are generated via the Hybrid Equations (HyEQ) Toolbox for MATLAB; see \cite{74}.
	Code available at https://github.com/HybridSystemsLab/InvariantBoucingBall.}
Over the simulation horizon, the disturbance $w_d$ is randomly generated within interval $[e_1, e_2]$ after each impact.
One solution that starts from the initial condition for $x$ given by $(11, 0)$ is shown in Figure~\ref{fig:bball1}.
Figure~\ref{fig:bball1}(a) presents the randomly generated $w_d$ disturbance for $\Huw$.
Moreover, even under uncertain disturbances, the peaks of the resulting height reach values larger than $\hmin$ and smaller than $\hmax$ as Figure~\ref{fig:bball1}(a) shows.
Figure~\ref{fig:bball1}(b) shows, on the $(x_1, x_2)$ plane, that solution stays within the set $\K$, which is the region bounded by dark green dashed line.

\IfConf{
\setlength{\unitlength}{0.28\textwidth}
}{
\setlength{\unitlength}{0.4\textwidth}}
\begin{figure}[H]
	\scriptsize
	\begin{subfigure}[t]{0.5\textwidth}
		\centering
		\includegraphics[trim = {0 4.5cm 0 0},clip,width = \unitlength]{sig1.eps}
		\put(-.02, .78){$\hmax$}
		\put(-.02, .74){$\hmin$}
		\put(-1.03, .7){$x_1$}
		\put(-1.03, .43){$x_2$}
		\put(-0.02, .26){$e_2$}
		\put(-0.02, .1){$e_1$}
		\put(-1.03, .18){$w_d$}
		\put(-.54, -.01){$t$ [sec]}
		\caption{Ball position and velocity and $w_d$.}
		\label{fig:sig1}
	\end{subfigure}
	\begin{subfigure}[t]{0.5\textwidth}
		\centering
		\includegraphics[trim = {0 4.5cm 0 0},clip,width = \unitlength]{sball1.eps}
		\put(-1.06,.43){$x_2$}
		\put(-.5,-.03){$x_1$}
%		\put(-30, 15){\vector(-1,1){10}}
		\put(-.2,.3){$\K$}
		\put(-.18,.46){(11,0)}
		\caption{Solution on the $(x_1, x_2)$ plane.}
		\label{fig:tball1}
	\end{subfigure}
	\caption{\label{fig:bball1} Simulation of $\Huw$ controlled by $\kd$ in \eqref{eq:Bkd}.}
\end{figure}
}

Next, using the results in Section~\ref{sec:rselect}, a control law with minimum point-wise norm rendering the set $\K$ in \eqref{eq:BK} robustly controlled forward invariant for $\Huw$ is provided.
Such a feedback is given by
$$\kmd (x) = \argmin\limits_{u_d \in \overline{S_d(x)}} |u_d|,$$
where $\overline{S_d(x)}$ is as in \eqref{eq:BSdcl} and it leads to the continuous feedback law
\begin{align}\label{eq:Brd}
	\kmd(x) = \max\left\{\sqrt{2\gamma \left(\frac{\varepsilon}{2} + \hmin\right)} + e_1x_2, 0\right\},
\end{align}
for every $x \in \K \cap \Pd{D_1}$.
Following same steps as above, it can be shown that $\K$ in \eqref{eq:BK} is robustly controlled forward invariant for $\Huw$ via $\kmd$ applying Corollary~\ref{coro:rcFI}.

Simulations are generated for $\Huw$ controlled by $\kmd$ given as in \eqref{eq:Brd} with the same system settings as above.
One solution that starts from the same initial condition $x = (11,0)$ is shown in Figure~\ref{fig:bball0}.
As shown in Figure~\ref{fig:bball0}(a), the peaks of the height in between impacts are between $\hmin = 10$ and $\hmax = 12$, while on the $(x_1, x_2)$ plane, the trajectory stays within the set $\K$, which is the region bounded by dark green dashed lines.

As expected, compared to Figure~\ref{fig:bball1}(a), we observe that there are only 7 impacts with the controlled surface within the time span of 0 to 20 seconds in Figure~\ref{fig:bball0}(a); while there are 14 impacts in Figure~\ref{fig:bball1}(a) and every impact is followed with a pull.
This indicates that less energy is used to bounce the ball at the controlled surface to maintain peak position within range $[\hmin, \hmax]$.
\begin{figure}[H]
	\scriptsize
	\begin{subfigure}[t]{0.5\textwidth}
		\centering
		\includegraphics[trim = {0 4cm 0 0},clip,width = \unitlength]{sig0.eps}
		\put(-.02, .78){$\hmax$}
		\put(-.02, .74){$\hmin$}
		\put(-1.03, .7){$x_1$}
		\put(-1.03, .43){$x_2$}
		\put(-0.02, .26){$e_2$}
		\put(-0.02, .1){$e_1$}
		\put(-1.03, .18){$w_d$}
		\put(-.54, -.01){$t$ [sec]}
		\caption{Ball position and velocity and $w_d$.}
		\label{fig:sig0}
	\end{subfigure}
	\begin{subfigure}[t]{0.5\textwidth}
		\centering
		\includegraphics[trim = {0 4.2cm 0 0},clip,width = \unitlength]{sball0.eps}
		\put(-1.06,.43){$x_2$}
		\put(-.5,-.03){$x_1$}
		\put(-.2,.2){$\K$}
		\put(-.2,.54){(11,0)}
		\put(-.14,.53){\line(1,-2){0.05}}
		\caption{Solution on the $(x_1, x_2)$ plane.}
		\label{fig:tball0}
	\end{subfigure}
	\caption{\label{fig:bball0} Simulation of $\Huw$ controlled by $\kmd$ in \eqref{eq:Brd}.}
\end{figure}
